Environment-Aware Minimum-Cost Wireless Backhaul Network Planning with Full-Duplex Links

In this work, we address the joint design of the wireless backhauling network topology as well as the frequency/power allocation on the wireless links, where nodes are capable of full-duplex (FD) operation. The proposed joint design enables the coexistence of multiple wireless links at the same channel, resulting in an enhanced spectral efficiency. Moreover, it enables the usage of FD capability when/where it is gainful. In this regard, a mixed-integer-linear-program (MILP) is proposed, aiming at a minimum cost design for the wireless backhaul network, considering the required rate demand at each base station. Moreover, a re-tunning algorithm is proposed which reacts to the slight changes in the network condition, e.g., channel attenuation or rate demand, by adjusting the transmit power at the wireless links. In this regard, a successive inner approximation (SIA)- based design is proposed, where in each step a convex subproblem is solved. Numerical simulations show a reduction in the overall network cost via the utilization of the proposed designs, thanks to the coexistence of multiple wireless links on the same channel due to the FD capability.

==> Sections/sec_abstract.tex <==
 In this paper we address a worst-case weighted sum rate maximization problem for a full-duplex (FD) and multi-carrier point-to-point (P2P) system. The effects of channel-state information (CSI) error, as well as the signal distortion due to hardware impairments are jointly taken into account. This also includes the inter-carrier destruction due to the non-linear distortions in a FD transceiver. Due to the non-tractable structure of the resulting problem, a weighted minimum mean squared error (WMMSE) method is applied to cast the rate maximization problem into a separately convex optimization problem, which can be iteratively solved with a guaranteed convergence to a local optimum. Moreover, a methodology to obtain the least favorable error matrices is proposed by casting the resulting non-convex quadratic optimization into a convex optimization problem. The achievable guaranteed (worst-case) rate is then numerically studied, over different levels of CSI error and transceiver accuracy.

